JMSNAS: Joint Model Split and Neural Architecture Search for Learning over Mobile Edge Networks

The main challenge to deploy deep neural network (DNN) over a mobile edge network is how to split the DNN model so as to match the network architecture as well as all the nodes' computation and communication capacity. This essentially involves two highly coupled procedures: model generating and model splitting. In this paper, a joint model split and neural architecture search (JMSNAS) framework is proposed to automatically generate and deploy a DNN model over a mobile edge network. Considering both the computing and communication resource constraints, a computational graph search problem is formulated to find the multi-split points of the DNN model, and then the model is trained to meet some accuracy requirements. Moreover, the trade-off between model accuracy and completion latency is achieved through the proper design of the objective function. The experiment results confirm the superiority of the proposed framework over the state-of-the-art split machine learning design methods.

==> _txt/7_Acknowledgment.tex <==
\section*{Acknowledgment}
This work was supported in part by National Key R\&D Program of China under Grant 2020YFB1807101, and National Natural Science Foundation of China under Grant U20A20158 and 61725104.

